CLIPRerank: An Extremely Simple Method for Improving Ad-hoc Video Search

Ad-hoc Video Search (AVS) enables users to search for unlabeled video content using on-the-fly textual queries. Current deep learning-based models for AVS are trained to optimize holistic similarity between short videos and their associated descriptions. However, due to the diversity of ad-hoc queries, even for a short video, its truly relevant part w.r.t. a given query can be of shorter duration. In such a scenario, the holistic similarity becomes suboptimal. To remedy the issue, we propose in this paper CLIPRerank, a fine-grained re-scoring method. We compute cross-modal similarities between query and video frames using a pre-trained CLIP model, with multi-frame scores aggregated by max pooling. The fine-grained score is weightedly added to the initial score for search result reranking. As such, CLIPRerank is agnostic to the underlying video retrieval models and extremely simple, making it a handy plug-in for boosting AVS. Experiments on the challenging TRECVID AVS benchmarks (from 2016 to 2021) justify the effectiveness of the proposed strategy. CLIPRerank consistently improves the TRECVID top performers and multiple existing models including SEA, W2VV++, Dual Encoding, Dual Task, LAFF, CLIP2Video, TS2-Net and X-CLIP. Our method also works when substituting BLIP-2 for CLIP.

==> analysis.tex <==
\input{table-sotas}
\subsection{Dose re-scoring by CLIP improve AVS ? }\label{does1}
 Our aim is to improve the initial rankings through an easily implementable re-scoring strategy. As demonstrated in \cref{tab:compare_sota}, following the implementation of re-scoring, the performance of all models has demonstrated noteworthy improvements, with the most substantial enhancement reaching an impressive 61.1\% ( $0.054 \rightarrow 0.087$), as observed in the case of the TV16 winning solution.
 In addition, with regard to the results obtained from TS2-Net, CLIP-FT, X-CLIP, and CLIP2Video, despite these models being initialized with trained CLIP parameters, their performance has surpassed that of using CLIP for zero-shot. Nevertheless, leveraging CLIP for frame-level similarity calculation and subsequent re-scoring still yields performance improvements. 
For example, CLIP2Video has shown an increase from 0.193 to 0.202 in overall performance on TV16-TV21, marking a performance improvement of 4.7\%. This indicates that a frame can also effectively characterize a short video thus complementing the video model with significant static information.
% In terms of overall performance on TRECVID 16-21, 
% static appearance
\subsection{Does MEA bring performance enhancements ?}
Compared with the LAFF and MEA from \cref{tab:compare_sota}, MEA improves the performance from 0.236 to 0.296 under the same features and training data. Based on the experimental design of the observation of \cite{li2022renmin}, MEA outperforms even the winning solutions of TV20 and TV21, which have much higher performance in previous experiments than the other up-to-date models. It is worth noting that the final submitted results of winner solutions are generally the results of multi-model fusion, whereas we report here only the results of the single-model MEA. 
 
\subsection{Does a more powerful VL model matter ?}
In the previous sections \ref{does1}, findings from our experimental results suggested that the re-scoring by CLIP is effective. Since the model for this re-scoring can be arbitrary, can we leverage a more powerful Vision-Language (VL) model to achieve further performance improvements? 
To test whether more powerful models can lead to better performance, we try \textit{CLIP-L/16@336}, which performs better than \textit{CLIP-B/32} on the overall performance of 27 datasets \footnote{\url{https://openai.com/research/clip}}, denoted as MEA-CLIP$^*$.  Shown as \cref{tab:compare_sota}, the performance improvement from 1.4\% to 6.6\%. Additionally, we set $k$ to 5000 to verify if more candidate video has an impact, compared MEA-CLIP$^*$ with  MEA-CLIP$^*$-5k, it also resulted in performance gains (from 6.6\% to 7.5\%). Compared MEA$^*$ with  MEA$^*$-CLIP$^*$-5k, although MEA$^*$ has achieved high performance compared to other models, after reranking, the performance still improves. According to \cite{li2022renmin}, we utilize BLIP-2 \footnote{\url{https://github.com/salesforce/LAVIS/tree/main/projects/blip2}}  for reranking MEA* on the latest V3C2 test set, achieving similar effectiveness. Specifically, $k$ is set to 5000, $\alpha $ is set to 0.1, and the performance is increased from 0.241 to 0.271. Per-query analysis on TV22 shows that there remain difficult queries that the re-scoring fails to respond, see \cref{fig:tv22}. 
As can be seen in the \cref{fig:tv22}, there is a slight decrease in queries \textit{\#705}, \textit{\#726}, \textit{\#727}, \textit{\#730}. Visual examination of the ranking outcomes for these queries reveals that the number of returned correct videos in the top 10 is approximate. Furthermore, it is noteworthy that a particularly challenging query, \textit{\#710: A person wearing a light t-shirt with dark or black writing on it}, initially exhibited an infAP of 0.0002 for the initial result. However, after applying reranking, this metric increased to 0.007. Visual examination of the retrieval results reveals that the original top 10 videos did not include any correct matches. Nevertheless, the effectiveness of the retrieval notably improved following the reranking process, as shown in \cref{fig:demo}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=1\columnwidth]{TV22_LAFF_BLIP}
    \caption{\textbf{ Per-query analysis on TV22}. 
}
    \label{fig:tv22}
\end{figure}

\begin{figure*}[htb!]
    \centering
    \includegraphics[width=2\columnwidth]{fig3_t10}
    \caption{\textbf{ Visualization of ranking list when apply rerank}. 
}
    \label{fig:demo}
\end{figure*}

% top10
% MEA
% 705 10
% 726 4
% 727 3
% 730 2
% BLIP2 rerank
% 705 9
% 726 3
% 727 5
% 730 3



% Vimeo Creative Commons Collection (V3C2) is 9760 videos (1.6 TB, 1300 total hours) with mean video duration of 8 min and total 1,425,454 video segments.

% . Chen \etal \cite{ChenHu2021} conducted a comprehensive analysis of the matters for Ad-hoc Video Search, and the study shows that features have a great impact on performance.

% 由于这个re-scoring的的model可以是任意的，利用更强大的模型，也能带来更好的性能，如我们尝试了在众多公共benchmark 上性能更好的CLIP-B/16 和CLIP-L/16@336. 由此可以见，可以尝试更多的图文模型，甚至text-to-video模型来进行re-scoing.




% \subsection{What role do features \& common space play in video retrieval ?}
% Chen \etal \cite{ChenHu2021} conducted a comprehensive analysis of the matters for Ad-hoc Video Search, and the study shows that features have a great impact on performance. So we try to improve SEA with the features used by the proposed new variant MEA, noted as SEA$^{*}$. Shown as \cref{tab:testsea}, we can find that incorporating a more relevant set of features can enhance model performance, however, the astute design of multi-modal alignment across various common spaces is also crucial.
% % \input{table-sea}
% \input{icassp2024/ICASSP/table_sota_cyy}

% \subsection{Dose a static representation enough? }\label{does2
% 从表格中的实验可以看出，CLIP的zero-shot 性能虽然W2VVPP的性能相当，但说明CLIP的zero-shot能力
% a strong static representation can also achieves much higher performance 
% the  grew from In addition, as shown as \cref{tab:compare_sota}, 
 % 如果只用CLIP 模型进行单一的相似度度量模型，性能远不如

 % From this, it is possible to experiment with larger pre-trained text-visual models and even text-to-video models for re-scoring

==> table-sea.tex <==



\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
\normalsize
\centering
\caption{\textbf{Comparison of the baseline SEA and improved variant MEA }.}
\label{tab:testsea}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{llllllll}
\toprule
Model    & \multicolumn{1}{l}{TV16} & \multicolumn{1}{l}{TV17} & \multicolumn{1}{l}{TV18} & \multicolumn{1}{l}{TV19} & \multicolumn{1}{l}{TV20} & \multicolumn{1}{l}{TV21}  & \multicolumn{1}{l}{MEAN} \\\hline
SEA
& \multicolumn{1}{r}{0.153} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.129} 
& \multicolumn{1}{r}{0.169} 
& \multicolumn{1}{r}{0.201} 
& \multicolumn{1}{r}{0.199}  
& \multicolumn{1}{r}{0.181} \\
SEA$^{*}$ 
& \multicolumn{1}{r}{0.192}
& \multicolumn{1}{r}{0.302}                    
& \multicolumn{1}{r}{0.169}                    
& \multicolumn{1}{r}{0.195}                    
& \multicolumn{1}{r}{0.331}                    
& \multicolumn{1}{r}{0.314}                                   
& \multicolumn{1}{r}{0.251} \\
MEA 
& \multicolumn{1}{r}{0.200}                    
& \multicolumn{1}{r}{0.313}                    
& \multicolumn{1}{r}{0.183}                    
& \multicolumn{1}{r}{0.214}                    
& \multicolumn{1}{r}{0.350}                    
& \multicolumn{1}{r}{0.342}                                      
& \multicolumn{1}{r}{0.267}  \\ \hline
\end{tabular}}
\end{center}
\end{table}

==> table-sotas.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \begin{tabular}{lrrrrrrr}
% & \multicolumn{1}{l}{TV16}         & \multicolumn{1}{l}{TV17}         & \multicolumn{1}{l}{TV18}         & \multicolumn{1}{l}{TV19}         & \multicolumn{1}{l}{TV20}         & \multicolumn{1}{l}{TV21}         & \multicolumn{1}{l}{MEAN}         \\
\begin{table*}[tbh!]
\caption{Comparison with the state-of-the-art}
\label{tab:compare_sota}
 \scalebox{0.9}{
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{1}{l}{Model} & \multicolumn{1}{r}{TV16} & \multicolumn{1}{r}{TV17} & \multicolumn{1}{r}{TV18} & \multicolumn{1}{r}{TV19}& \multicolumn{1}{r}{TV20} & \multicolumn{1}{r}{TV21} & \multicolumn{1}{r}{MEAN} \\ 
\hline
Winning solutions                                  
& \multicolumn{1}{r}{0.054 \cite{tv16-TOP1}} 
& \multicolumn{1}{r}{0.206 \cite{tv17-TOP1}} 
& \multicolumn{1}{r}{0.121  \cite{tv18-TOP1}} 
& \multicolumn{1}{r}{0.163  \cite{tv19-TOP1}} 
& \multicolumn{1}{r}{0.354  \cite{tv20-TOP1}} 
& \multicolumn{1}{r}{0.355  \cite{tv21-TOP1}}
& \multicolumn{1}{r}{--} \\ 
DualTask\cite{wu2020interpretable_dual_task}
& \multicolumn{1}{r}{0.185} 
& \multicolumn{1}{r}{0.241} 
& \multicolumn{1}{r}{0.123} 
& \multicolumn{1}{r}{0.185} 
& \multicolumn{1}{r}{--} 
& \multicolumn{1}{r}{--}
& \multicolumn{1}{r}{--} \\
W2VV++ \cite{LiXirong2019W2VVPP} 
& \multicolumn{1}{r}{0.162} 
& \multicolumn{1}{r}{0.223} 
& \multicolumn{1}{r}{0.101} 
& \multicolumn{1}{r}{0.139} 
& \multicolumn{1}{r}{0.163} 
& \multicolumn{1}{r}{0.137} 
& \multicolumn{1}{r}{0.154}  \\
CLIP-pre \cite{ChenHu2021}
& \multicolumn{1}{r}{0.173}
& \multicolumn{1}{r}{0.202} 
& \multicolumn{1}{r}{0.092} 
& \multicolumn{1}{r}{0.124} 
& \multicolumn{1}{r}{0.134} 
& \multicolumn{1}{r}{0.197} 
& \multicolumn{1}{r}{0.154} \\

TS2-NET \cite{liu2022ts2net}
& \multicolumn{1}{r}{0.191}
& \multicolumn{1}{r}{0.245} 
& \multicolumn{1}{r}{0.112} 
& \multicolumn{1}{r}{0.120} 
& \multicolumn{1}{r}{0.153} 
& \multicolumn{1}{r}{0.188} 
& \multicolumn{1}{r}{0.168} \\
Dual Encoding \cite{cvpr19-zevr} 
& \multicolumn{1}{r}{0.163 } 
& \multicolumn{1}{r}{0.228 } 
& \multicolumn{1}{r}{0.116} 
& \multicolumn{1}{r}{0.164} 
& \multicolumn{1}{r}{0.186}
& \multicolumn{1}{r}{0.166} 
& \multicolumn{1}{r}{0.170 }  \\
CLIP-FT \cite{hu2021lightweight_LAFF} 
& \multicolumn{1}{r}{0.191}
& \multicolumn{1}{r}{0.215} 
& \multicolumn{1}{r}{0.105} 
& \multicolumn{1}{r}{0.147} 
& \multicolumn{1}{r}{0.203} 
& \multicolumn{1}{r}{0.208} 
& \multicolumn{1}{r}{0.178}  \\
X-CLIP \cite{xclip} 
& \multicolumn{1}{r}{0.209}
& \multicolumn{1}{r}{0.229} 
& \multicolumn{1}{r}{0.114} 
& \multicolumn{1}{r}{0.150} 
& \multicolumn{1}{r}{0.184} 
& \multicolumn{1}{r}{0.195} 
& \multicolumn{1}{r}{0.180}  \\
SEA \cite{LiXirong2020SEA} 
& \multicolumn{1}{r}{0.153} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.129} 
& \multicolumn{1}{r}{0.169} 
& \multicolumn{1}{r}{0.201} 
& \multicolumn{1}{r}{0.199}  
& \multicolumn{1}{r}{0.181} \\
CLIP2Video \cite{fang2021clip2video} 
& \multicolumn{1}{r}{0.176} 
& \multicolumn{1}{r}{0.229} 
& \multicolumn{1}{r}{0.114} 
& \multicolumn{1}{r}{0.176} 
& \multicolumn{1}{r}{0.207} 
& \multicolumn{1}{r}{0.255} 
& \multicolumn{1}{r}{0.193}  \\
LAFF \cite{hu2021lightweight_LAFF} 
& \multicolumn{1}{r}{0.211} 
& \multicolumn{1}{r}{0.285} 
& \multicolumn{1}{r}{0.137} 
& \multicolumn{1}{r}{0.192} 
& \multicolumn{1}{r}{0.265} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.221}  \\
MEA  	 	 	 
& \multicolumn{1}{r}{0.216 } 
& \multicolumn{1}{r}{0.313} 
& \multicolumn{1}{r}{0.147 } 
& \multicolumn{1}{r}{0.206} 
& \multicolumn{1}{r}{0.297} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.236}  \\
MEA* 
& \multicolumn{1}{r}{0.262} 
& \multicolumn{1}{r}{0.357} 
& \multicolumn{1}{r}{0.192} 
& \multicolumn{1}{r}{0.243} 
& \multicolumn{1}{r}{0.358} 
& \multicolumn{1}{r}{0.361} 
& \multicolumn{1}{r}{0.296}  \\

\midrule
\multicolumn{8}{l}{\textbf{\textit{with Re-scoring}}}  \\ 
Winner solutions 
& 0.087 (61.1\%) 
& 0.247 (19.1\%) 
& 0.143 (18.2\%) 
& 0.192 (17.8\%) 
& 0.372 (5.1\%) 
& 0.361 (1.7\%) 
& -- \\ 
DualTask
& 0.214  (15.6\%) 
& 0.277  (14.8\%) 
& 0.142  (14.7\%) 
& 0.210  (13.6\%) 
& -- 
& -- 
& -- \\
CLIP-pre
& 0.170  (-1.4\%) 
& 0.209  (3.4\%) 
& 0.094  (1.6\%) 
& 0.124  (-0.1\%)
& 0.136  (1.0\%) 
& 0.201  (1.8\%) 
& 0.155  (1.1\%)  \\
TS2-NET
& 0.196  (2.6\%)
& 0.258  (5.3\%) 
& 0.114  (1.8\%)
& 0.124  (3.3\%)
& 0.157  (2.6\%)
& 0.192  (2.1\%)
& 0.173  (3.0\%) \\
W2VV++ 
& 0.204  (26.1\%)
& 0.260  (16.5\%) 
& 0.126  (24.9\%) 
& 0.168  (21.1\%) 
& 0.181  (11.1\%) 
& 0.160  (17.3\%) 
& 0.183  (19.0\%) \\

CLIP-FT
& 0.189  (3.3\%)
& 0.236  (8.3\%) 
& 0.109  (1.9\%)
& 0.154  (7.7\%)
& 0.205  (2.0\%) 
& 0.213  (2.0\%)
& 0.184  (4.0\%)  \\

X-CLIP				
& 0.214  (2.4\%)
& 0.235  (2.6\%)
& 0.117  (2.6\%)
& 0.156  (4.0\%)
& 0.188  (2.2\%)
& 0.199  (2.1\%)
& 0.185  (2.8\%)  \\
Dual Encoding
& 0.197  (20.8\%)	
& 0.267  (17.1\%)
& 0.133  (14.9\%)	
& 0.189  (15.5\%)	
& 0.207  (11.0\%)	
& 0.185  (11.6\%)	
& 0.196  (15.2\%) \\
CLIP2Video 
& 0.186  (5.5\%) 
& 0.242  (5.5\%)
& 0.119  (3.9\%) 
& 0.187  (6.3\%) 
& 0.214  (3.5\%) 
& 0.264  (3.7\%) 
& 0.202  (4.7\%) \\
SEA 
& 0.196  (28.0\%)	
& 0.270  (14.7\%)	
& 0.149  (15.8\%)	
& 0.196  (16.1\%)	
& 0.223  (10.8\%)	
& 0.220  (10.4\%)	
& 0.209  (15.4\%) \\

LAFF
& 0.216  (2.5\%) 
& 0.293  (2.8\%) 
& 0.149  (8.9\%) 
& 0.194  (1.2\%) 
& 0.266  (0.3\%) 
& 0.236  (0.3\%)
& 0.226  (2.1\%)  \\
				
MEA					
& 0.221  (2.5\%)
& 0.318  (1.7\%)
& 0.150  (1.7\%)
& 0.208  (1.1\%)
& 0.300  (1.1\%)
& 0.237  (0.9\%)
& 0.239  (1.4\%)  \\
					
MEA-CLIP$*$ 						
& 0.242  (11.8\%)
& 0.324  (3.4\%)
& 0.167  (13.7\%)
& 0.216  (4.6\%)
& 0.300  (1.1\%)
& 0.259  (10.1\%)
& 0.252  (6.6\%)  \\

MEA-CLIP$*$-5k 						
& 0.250  (15.6\%)
& 0.336  (7.2\%)
& 0.163  (10.6\%) 
& 0.213  (3.6\%)
& 0.303  (2.2\%)
& 0.255  (8.4\%)
& 0.254  (7.5\%)  \\

MEA$*$-CLIP$*$-5k 						
& 0.282  (7.6\%)
& 0.368  (3.1\%)
& 0.197  (2.6\%)
& 0.255  (4.9\%)
& 0.361  (0.8\%)
& 0.365  (1.1\%)
& 0.305  (3.4\%)  \\

% LAFF
% & 0.222  (5.4\%) 
% & 0.289  (1.3\%) 
% & 0.150  (10.0\%) 
% & 0.212  (10.0\%) 
% & 0.274  (3.7\%) 
% & 0.253  (7.5\%) 
% & 0.233  (6.3\%)  \\
						
% MEA 						
% & 0.222  (11.0\%) 
% & 0.330  (5.4\%)
% & 0.185  (1.1\%) 
% & 0.224  (4.7\%)
% & 0.352  (0.6\%)
% & 0.342  (0.0\%)
% & 0.276  (3.4\%)  \\

% MEA-CLIP$*$ 						
% & 0.233  (16.5\%)
% & 0.335  (7.0\%)
% & 0.191  (4.4\%) 
% & 0.226  (5.6\%)
% & 0.353  (0.9\%)
% & 0.351  (2.6\%)
% & 0.282  (5.6\%)  \\

% MEA-CLIP$*$-5k 						
% & 0.245  (22.5\%)
% & 0.353  (12.8\%)
% & 0.189  (3.3\%)
% & 0.234  (9.3\%)
% & 0.357  (2.0\%)
% & 0.349  (2.0\%)
% & 0.288  (7.9\%)  \\




\bottomrule
\end{tabular}
}
\end{table*}

==> table-sotas_bk.tex <==
\begin{table*}[tbh!]
\caption{Comparison with the state-of-the-art}
\label{tab:compare_sota}
 \scalebox{0.9}{
\begin{tabular}{llllllll}
\toprule
Model & TV16 & TV17 & TV18 & TV19c& TV20 & TV21 & MEAN \\ 
\hline
Winner solutions
& \multicolumn{1}{r}{0.054 \cite{tv16-TOP1}} 
& \multicolumn{1}{r}{0.206 \cite{tv17-TOP1}} 
& \multicolumn{1}{r}{0.121  \cite{tv18-TOP1}} 
& \multicolumn{1}{r}{0.163  \cite{tv19-TOP1}} 
& \multicolumn{1}{r}{0.354  \cite{tv20-TOP1}} 
& \multicolumn{1}{r}{0.355  \cite{tv21-TOP1}}
& \multicolumn{1}{r}{--} \\ 
W2VV++ \cite{LiXirong2019W2VVPP} 
& \multicolumn{1}{r}{0.162} 
& \multicolumn{1}{r}{0.223} 
& \multicolumn{1}{r}{0.101} 
& \multicolumn{1}{r}{0.139} 
& \multicolumn{1}{r}{0.163} 
& \multicolumn{1}{r}{0.137} 
& \multicolumn{1}{r}{0.154}  \\
DualTask\cite{wu2020interpretable_dual_task}
& \multicolumn{1}{r}{0.185} 
& \multicolumn{1}{r}{0.241} 
& \multicolumn{1}{r}{0.123} 
& \multicolumn{1}{r}{0.185} 
& \multicolumn{1}{r}{--} 
& \multicolumn{1}{r}{--}
& \multicolumn{1}{r}{--} \\
CLIP-pre \cite{ChenHu2021}
& \multicolumn{1}{r}{0.173}
& \multicolumn{1}{r}{0.202} 
& \multicolumn{1}{r}{0.092} 
& \multicolumn{1}{r}{0.124} 
& \multicolumn{1}{r}{0.134} 
& \multicolumn{1}{r}{0.197} 
& \multicolumn{1}{r}{0.154} \\
Dual Encoding \cite{cvpr19-zevr} 
& \multicolumn{1}{r}{0.163 } 
& \multicolumn{1}{r}{0.228 } 
& \multicolumn{1}{r}{0.116} 
& \multicolumn{1}{r}{0.164} 
& \multicolumn{1}{r}{0.186}
& \multicolumn{1}{r}{0.166} 
& \multicolumn{1}{r}{0.170 }  \\
CLIP-FT \cite{hu2021lightweight_LAFF} 
& \multicolumn{1}{r}{0.191}
& \multicolumn{1}{r}{0.215} 
& \multicolumn{1}{r}{0.105} 
& \multicolumn{1}{r}{0.147} 
& \multicolumn{1}{r}{0.203} 
& \multicolumn{1}{r}{0.208} 
& \multicolumn{1}{r}{0.178}  \\
SEA \cite{LiXirong2020SEA} 
& \multicolumn{1}{r}{0.153} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.129} 
& \multicolumn{1}{r}{0.169} 
& \multicolumn{1}{r}{0.201} 
& \multicolumn{1}{r}{0.199}  
& \multicolumn{1}{r}{0.181} \\

CLIP2Video \cite{fang2021clip2video} 
& \multicolumn{1}{r}{0.176} 
& \multicolumn{1}{r}{0.229} 
& \multicolumn{1}{r}{0.114} 
& \multicolumn{1}{r}{0.176} 
& \multicolumn{1}{r}{0.207} 
& \multicolumn{1}{r}{0.255} 
& \multicolumn{1}{r}{0.193}  \\
LAFF \cite{hu2021lightweight_LAFF} 
& \multicolumn{1}{r}{0.211} 
& \multicolumn{1}{r}{0.285} 
& \multicolumn{1}{r}{0.137} 
& \multicolumn{1}{r}{0.192} 
& \multicolumn{1}{r}{0.265} 
& \multicolumn{1}{r}{0.235} 
& \multicolumn{1}{r}{0.221}  \\
this paper
& \multicolumn{1}{r}{0.200} 
& \multicolumn{1}{r}{0.313} 
& \multicolumn{1}{r}{0.183} 
& \multicolumn{1}{r}{0.214} 
& \multicolumn{1}{r}{0.350} 
& \multicolumn{1}{r}{0.342} 
& \multicolumn{1}{r}{0.267}  \\
\midrule
\multicolumn{8}{l}{\textbf{\textit{with Re-scoring}}}  \\ 
Winner solutions 
& 0.087 (61.1\%) 
& 0.247 (19.1\%) 
& 0.143 (18.2\%) 
& 0.192 (17.8\%) 
& 0.372 \space\space(5.1\%) 
& 0.361 \space\space(1.7\%) 
& -- \\
Dual Encoding
& 0.197  (20.8\%)	
& 0.267  (17.1\%)
& 0.133  (14.9\%)	
& 0.189  (15.5\%)	
& 0.207  (11.0\%)	
& 0.185  (11.6\%)	
& 0.196  (15.2\%) \\
W2VV++ 
& 0.204  (26.1\%)
& 0.260  (16.5\%) 
& 0.126  (24.9\%) 
& 0.168  (21.1\%) 
& 0.181  (11.1\%) 
& 0.160  (17.3\%) 
& 0.183  (19.0\%) \\
DualTask
& 0.214  (15.6\%) 
& 0.277  (14.8\%) 
& 0.142  (14.7\%) 
& 0.210  (13.6\%) 
& -- 
& -- 
& -- \\
SEA 
& 0.196  (28.0\%)	
& 0.270  (14.7\%)	
& 0.149  (15.8\%)	
& 0.196  (16.1\%)	
& 0.223  (10.8\%)	
& 0.220  (10.4\%)	
& 0.209  (15.4\%) \\
LAFF
& 0.222  \space\space(5.4\%) 
& 0.289  \space\space(1.3\%) 
& 0.150  (10.0\%) 
& 0.212  (10.0\%) 
& 0.274  \space\space(3.7\%) 
& 0.253  \space\space(7.5\%) 
& 0.233  \space\space(6.3\%)  \\
CLIP-pre
& 0.170  \space(-1.4\%) 
& 0.209  \space\space(3.4\%) 
& 0.094  \space\space(1.6\%) 
& 0.124  \space(-0.1\%)
& 0.136  \space\space(1.0\%) 
& 0.201  \space\space(1.8\%) 
& 0.155  \space\space(1.1\%)  \\
CLIP-FT 
& 0.207  \space\space(8.3\%) 
& 0.242  (12.6\%) 
& 0.122  (16.6\%) 
& 0.164  (11.8\%) 
& 0.214  \space\space(5.0\%) 
& 0.226  \space\space(8.6\%) 
& 0.196  (10.5\%)  \\
CLIP2Video 
& 0.186  \space\space(5.5\%) 
& 0.242  \space\space(5.5\%)
& 0.119  \space\space(3.9\%) 
& 0.187  \space\space(6.3\%) 
& 0.214  \space\space(3.5\%) 
& 0.264  \space\space(3.7\%) 
& 0.202  \space\space(4.7\%) \\
this paper
& 0.220 \space\space(9.9\%)				
& 0.325 \space\space(3.8\%)		
& 0.189 \space\space(3.5\%)	
& 0.228 \space\space(6.6\%)	
& 0.356 \space\space(1.6\%)	
& 0.346 \space\space(1.3\%)	
& 0.277 \space\space(4.4\%)	\\
\bottomrule
\end{tabular}
}
\end{table*}
